ZKFault: Fault attack analysis on zero-knowledge based post-quantum digital signature schemes

Computationally hard problems based on coding theory, such as the syndrome decoding problem, have been used for constructing secure cryptographic schemes for a long time. Schemes based on these problems are also assumed to be secure against quantum computers. However, these schemes are often considered impractical for real-world deployment due to large key sizes and inefficient computation time. In the recent call for standardization of additional post-quantum digital signatures by the National Institute of Standards and Technology, several code-based candidates have been proposed, including LESS, CROSS, and MEDS. These schemes are designed on the relatively new zero-knowledge framework. Although several works analyze the hardness of these schemes, there is hardly any work that examines the security of these schemes in the presence of physical attacks. In this work, we analyze these signature schemes from the perspective of fault attacks. All these schemes use a similar tree-based construction to compress the signature size. We attack this component of these schemes. Therefore, our attack is applicable to all of these schemes. In this work, we first analyze the LESS signature scheme and devise our attack. Furthermore, we showed how this attack can be extended to the CROSS signature scheme. Our attacks are built on very simple fault assumptions. Our results show that we can recover the entire secret key of LESS and CROSS using as little as a single fault. Finally, we propose various countermeasures to prevent these kinds of attacks and discuss their efficiency and shortcomings.

==> Appendices/Definitions.tex <==
\section{Some Definitions}
\begin{definition}[{Information Set (IS) of a Linear Code (\texttt{RREF} version)~\cite{A_New_Formulation_of_the_Linear_Equivalence_Problem}}]
Let $\code{C}$ be a linear code with length $n$, and $J\subset \ring{Z}{n}$ be a set with cardinality $k$. Consider $\mat{G}$ as the generator matrix of code $\code{C}$. Define $J$ as an information set corresponding to $\mat{G}$ if the equality  $\texttt{RREF}(\mat{G})=\mat{G}[*, J]^{-1}\mat{G}$ holds.
\end{definition}
\begin{definition}[{IS-Linear Equivalence (\texttt{RREF} version)~\cite{A_New_Formulation_of_the_Linear_Equivalence_Problem}}]
 Let $\mat{G}$ and $\mat{G}'$ be two generators of the linear codes 
$\code{C}$ and $\code{C}'$ respectively of length $n$ and dimension $k$. Then, we say $\code{C}$ and $\code{C}'$ are IS-Linear Equivalent if there exists an IS $J\subset \ring{Z}{n}$ of cardinality $k$, $\mat{Q}\in M_{n}$ and $\overline{\mat{Q}}\in \textit{M}_{n-k}'$ such that the following equality holds
\begin{align*}
&\widetilde{\mat{G}}[*,\ J]^{-1}\widetilde{\mat{G}}[*,\ J^{c}]=\mat{G}'[*,\ J]^{-1}\mat{G}'\overline{\mat{Q}}    
\end{align*}
where $\widetilde{\mat{G}}=\mat{GQ}$.  Consequently, The IS-Linear Equivalence Problem (IS-LEP) is: given two linear codes $\code{C}$ and $\code{C}'$, determine whether $\code{C}$ is IS-LEP to $\code{C}'$ or not.
\end{definition}

==> Appendices/Lemma.tex <==
\subsection{Probability of getting effective-faulted signature}\label{sec:ProbabilityEffectiveFault}



Before we start, recall that, $\vecentry{x}{2l-1},\ \vecentry{x}{2l},\ \cdots,\ \vecentry{x}{4l-2}$ are all the leaf nodes of the \textit{Reference Tree} $\vect{x}$. Let $\vecentry{x}{i}$ be the node in \textit{Reference Tree} with height $h$, and $L_{\vecentry{x}{i}}$ be the set of all leaf nodes of the subtree rooted at $\vecentry{x}{i}$. We only need the leaf nodes from $L_{\vecentry{x}{i}}$ that coincide with the first $t$ many leaf nodes of the full \textit{Reference Tree}. Let there be $v$ many such leaves, and let the set of indices of these leaves be 
$$I^{(i)}_{\text{leaf}} = \{j_1,\ j_2,\ \cdots,\ j_v\}\,.$$ 
This is the set corresponding to the node $\vecentry{x}{i}$.
%We call it as "effective leaves" of $\vecentry{x}{i}$. 
%Now, we will prove the following 
\begin{lemma}\label{lemma:effective-fault }
    If fault injection at the node $\vecentry{x}{i}$ is successful, then the probability that the fault is an "effective-fault" is 
$$\begin{cases}
1- \prod\limits_{j=0}^{v}\left(1-\frac{w}{t-j}\right) & \text{if } w>v\\
1-\prod\limits_{j=0}^{w-1}\left(\frac{v-j}{t-j}\right)-\prod\limits_{j=0}^{v}\left(1-\frac{w}{t-j}\right) & \text{otherwise}
\end{cases}$$
where $v = |I^{(i)}_{\text{leaf}}|$
%where $v$ is the number of effective leaves of $\vecentry{x}{i}$. 
\end{lemma}

\begin{proof} 
We assume the fault is successful, i.e., the instruction $Ins(i)$ has been skipped. Since all the values of the \textit{Reference Tree} $\vect{x}$ is initialized by zero, after successful-fault, the faulted \textit{Reference Tree} be $\vect{x'}$ and $\vecentry{x'}{i}=0$. Here, the following three cases may arise:\\ 
    
     \textbf{Case 1:} $\vecentry{x}{i}=0$ in non-faulted case. As we have already established, if $\vecentry{x}{i}$ is already zero, then changing its value would not mount an attack, so it is an ineffective-fault case. Now, we will find the probability of occurrence in this case, i.e., $\Pr\left[\vecentry{x}{i}=0\right]$. Now, 
    \begin{align*}
        \vecentry{x}{i}=0&\iff \text{ all the leaf nodes of the subtree rooted at }\vecentry{x}{i} \text{ are valued zero} \\
        &\iff\vecentry{x}{j}=0 ~\forall~ j\in I^{(i)}_{\text{leaf}}\iff\vecentry{f}{j-2l+1}=0 ~\forall~ j\in I^{(i)}_{\text{leaf}}\\
        &\iff\vecentry{d}{j-2l+1}=0 ~\forall~ j\in I^{(i)}_{\text{leaf}}
    \end{align*}
    Since the fixed digest vector $\vect{d}\in \ring{Z}{s}^{t}$ is an arbitrary vector of length $t$ and weight $w$, respectively, therefore the total number of all such possible vectors is $\binom{t}{w}\cdot (s-1)^w$. Also, the number of such vectors $\vect{d}$ such that the elements in the positions $\{j-2l+1:~j\in I^{(i)}_{\text{leaf}}\}$ are zero is $\binom{t-v}{w}\cdot (s-1)^w$. Therefore 
    %implies that all the  $\vecentry{d}{j-2l+1}=0$ for all $j\in I^{(i)}_{\text{leaf}}$. This case implies that all leaves of the subtree rooted at $\vecentry{x}{i}$ is zero, \textit{i.e.} $\vecentry{x}{i}=0$. As we have already established, if $\vecentry{x}{i}$ is already zero, then changing its value would not mount an attack. However, the probability that this case will occur is
    \begin{align*}
       \Pr[\vecentry{x}{i}=0]~=~ \frac{\binom{t-v}{w}\cdot (s-1)^w}{\binom{t}{w}\cdot (s-1)^w}~=~ \prod\limits_{j=0}^{v}\left(1-\frac{w}{t-j}\right) 
    \end{align*}
    \textbf{Case 2:} $\vecentry{x}{i}=1$ in the non-faulted case, and after successful fault injection $\vecentry{x'}{0}=0$. As we have already established, in this case also, we can not get information about the secret, so it is an ineffective-fault case. Now, we will find the probability of occurrence of this case, i.e., $\Pr[\vecentry{x}{i}=1 \text{ and }\vecentry{x'}{0}=0]$. 
    
    Now, $\vecentry{x}{i}=1 \text{ and }\vecentry{x'}{0}=0$ implies that all the leaf nodes with non-zero values have indices in the set $I^{(i)}_{\text{leaf}}$, otherwise $\vecentry{x'}{0}$ would have been $1$. i.e.,
    \begin{align*}
        \vecentry{x}{i}=1 \text{ and }\vecentry{x'}{0}=0&\iff \vecentry{x}{j}=0 ~\forall~ j\notin I^{(i)}_{\text{leaf}}\iff\vecentry{f}{j-2l+1}=0 ~\forall~ j\notin I^{(i)}_{\text{leaf}}\\
        &\iff\vecentry{d}{j-2l+1}=0 ~\forall~ j\notin I^{(i)}_{\text{leaf}}
    \end{align*}
    Now, $\vect{d}$ is a fixed weight vector in $\ring{Z}{s}^{t}$ with $wt(\vect{d})=w$. If $w>v$ then there must exist some $j\in I^{(i)}_{\text{leaf}}$ such that $\vecentry{d}{j-2l+1}\neq 0$. Therefore the number of vectors $\vect{d}$ such that $\vecentry{d}{j-2l+1}=0 ~\forall~ j\notin I^{(i)}_{\text{leaf}}$ is
    $$\begin{cases}
        0 & \text{if } w>v\\
        \binom{v}{w}\cdot (s-1)^w & \text{otherwise}
    \end{cases}$$
    
    %Now, the number of such vectors $\vect{d}\in \ring{Z}{s}^{t}$ such that the weight of $\vect{d}$ is $w$ and the elements in the positions $\{j-2l+1:~j\notin I_\text{leaf}\}$ are zero\\
    %= $|\{\vect{d}\in\ring{Z}{s}^{t}:~ wt(\vect{d})= w \text{ and }\vecentry{d}{j-2l+1}=0, \forall j\notin I^{(i)}_{\text{leaf}}\}|$\\
    %$
    %=|\{\vect{d_{1}}=(\vecentry{d}{j_{1}-2l+1},\ \cdots,\ \vecentry{d}{j_{v}-2l+1} )\in\ring{Z}{s}^{v}:~ wt(\vect{d_{1}})= w \}|=\begin{cases}
%0 & \text{if } w>v\\
%\binom{v}{w}\cdot (s-1)^w & \text{otherwise}
%\end{cases}$ 
Therefore,
   \begin{align*}
        \Pr[\vecentry{x}{i}=1 \text{ and }\vecentry{x'}{0}=0]
        &=\begin{cases}
0 & \text{if } w>v\\
\frac{\binom{v}{w}\cdot (s-1)^w}{\binom{t}{w}\cdot (s-1)^w} & \text{otherwise}
\end{cases}\\
&=\begin{cases}
0 & \text{if } w>v\\
\prod\limits_{i'=0}^{w-1}\left(\frac{v-i'}{t-i'}\right) & \text{otherwise}
\end{cases}  
    \end{align*}
    \textbf{Case 3:} $\vecentry{x}{i}=1$ in the non-faulted case, and after successful fault injection $\vecentry{x'}{0}=1$. As we have already established, in this case, we can get information about the secret, so it is an effective fault case. Since $\vecentry{x}{i}=1$, there exists some $j\in I^{(i)}_{\text{leaf}}$ such that $\vecentry{x}{j}=1$, i.e., $\vecentry{f}{j-2l+1}=1\implies\vecentry{d}{j-2l+1}\neq 0$. Also, since $\vecentry{x'}{0}=1$, there exists some $j'\notin I^{(i)}_{\text{leaf}}$ such that $\vecentry{x}{j'}=1$, i.e.,$\vecentry{f}{j'-2l+1}=1\implies \vecentry{d}{j'-2l+1}\neq 0$. The probability of this case occurs when neither \textbf{Case 1} nor \textbf{Case 2} occur, which is 
   $$\begin{cases}
1- \prod\limits_{i'=0}^{v}\left(1-\frac{w}{t-i'}\right) & \text{if } w>v\\
1-\prod\limits_{i'=0}^{w-1}\left(\frac{v-i'}{t-i'}\right)-\prod\limits_{i'=0}^{v}\left(1-\frac{w}{t-i'}\right) & \text{otherwise}
\end{cases}$$
This is the probability of effective fault.
\end{proof}

%  Since the products $\prod\limits_{i'=0}^{v}\left(1-\frac{w}{t-i'}\right)$ and $\prod\limits_{i'=0}^{w-1}\left(\frac{v-i'}{t-i'}\right)$  decrease in the time of $v$ increases, therefore 

%
Here, we want to get as much as possible secret information from one effective faulted signature. This will work if we can get multiple pairs $(\widetilde{\mat{Q}}_{k'},\ \mat{Q}_{\vecentry{d}{k'}}^{T}\overline{{\mat{Q}}}_{k'})$. So, we need a large number of non-zero leaf nodes of the subtree rooted at $\vecentry{x}{i}$ because then only we will get such multiple pairs from an effective faulted signature. Now, $\vecentry{x}{0}$ is the node having maximum leaf nodes, but in this case the fault will not be effective as after fault injection $\vecentry{x'}{0}$ will be zero. For this reason, we will select the node $\vecentry{x}{1}$.  %From Lemma~\ref{lemma:effective-fault }, it is evident that if $v$ increases, the probability that a successful fault is an "effective-fault" increases, where $v\geq w$. The value of $v$ depends on two things. First, the height of the node $\vecentry{x}{i}$ and second, the number of leaf nodes of the subtree rooted at $\vecentry{x}{i}$, that lies among the first $t$ many leaves of the \textit{Reference Tree} $\vect{x}$. Keeping both cases in mind, we have the maximum probability of "effective-fault" in the case where we inject fault at the node $\vecentry{x}{1}$. 
So, if the fault injection at the node $\vecentry{x}{1}$ is successful, then the probability that the fault is an "effective-fault" is $1-\prod\limits_{i'=0}^{w-1}\left(\frac{l-i'}{t-i'}\right)-\prod\limits_{i'=0}^{l}\left(1-\frac{w}{t-i'}\right)$, where $l=|I^{(1)}_{\text{leaf}}|$. Therefore the probability that the fault is an "effective-fault" is at least $\left(1-\prod\limits_{i'=0}^{w-1}\left(\frac{l-i'}{t-i'}\right)-\prod\limits_{i'=0}^{l}\left(1-\frac{w}{t-i'}\right)\right)\times p$, where $p=\Pr[\text{"successful-fault"}]$.


==> Appendices/Properties.tex <==
\section{Properties of monomial matrices}\label{appendix:properties}


\noindent\textbf{Some properties:}
Let $\mat{A}=(\pi,\ \vect{u})\in M_{n}(q)$ be a invertible monomial matrix. Then, the following properties holds: %$\mat{B}=(\pi',\ \vect{u'})\in M_{n}$, $\mat{C}=(\pi_{*},\ \vect{v})\in M_{k}'$. Then the important computational actions of monomial matrices are as follows: 

\begin{enumerate}
    \item $\matentry{A}{\pi(j)}{j}=\vecentry{u}{j}$ is the only non-zero element of the $j$-th column of $\mat{A}$.\label{properties:Non-zeroElement}
    \item The transpose of the matrix $\mat{A}$ is given by 
    $$\mat{A}^{T}=(\vecentry{u}{\pi^{-1}(0)}\basisvec{\pi^{-1}(0)}~|~\cdots~|~\vecentry{u}{\pi^{-1}(n-1)}\basisvec{\pi^{-1}(n-1)})$$\label{properties:Transpose}
    \item The multiplication of any matrix $\mat{G}$ with the monomial matrix $\mat{A}$ is given by
    $$\mat{GA}=(\vecentry{u}{0}\vect{g}_{\pi(0)}~|~\cdots~|~\vecentry{u}{n-1}\vect{g}_{\pi(n-1)})$$
where $\vect{g}_{j}=\matcol{G}{j}$ is the $j$-th column of the matrix $\mat{G}$.\label{properties:Multiplication}
    \item Let $\mat{B}=(\pi', \vect{u'})\in M_n(q)$, then the multiplication of two monomial matrices $\mat{A}$ and $\mat{B}$ is given by:
    $$\mat{AB}=(\vecentry{u}{\pi'(0)}\vecentry{u'}{0}\basisvec{\pi(\pi'(0))}~|~\cdots~|~\vecentry{u}{\pi'(n-1)}\vecentry{u'}{n-1}\basisvec{\pi(\pi'(n-1))})$$\label{properties:Mono-Multiplication}
    \item The multiplication of a monomial matrices $\mat{A}$ by a partial monomial matrix $\mat{C}=(\pi_{*},\ \vect{v})\in M_{k}'(q)$ is given by:
    $$\mat{AC}=(\vecentry{u}{\pi_{*}(0)}\vecentry{v}{0}\basisvec{\pi(\pi_{*}(0))}~|~\cdots~|~\vecentry{u}{\pi_{*}(k-1)}\vecentry{v}{k-1}\basisvec{\pi(\pi_{*}(k-1))})$$\label{properties:Mono-PartialMono-Multiplication}
\end{enumerate}
\noindent\textbf{Property 1: }$\matentry{A}{\pi(j)}{j}=\vecentry{u}{j}$ is the only non-zero element of $\pi(j)$-th row as well as $j$-th column of $\mat{A}$.

Here $\mat{A}=(\vecentry{u}{0}\basisvec{\pi(0)}~|~\cdots~|~\vecentry{u}{n-1}\basisvec{\pi(n-1)})$. So, the $j$-th column of $\mat{A}$ is $\matcol{A}{j}=\vecentry{u}{j}\basisvec{\pi(j)}$. Since $\basisvec{\pi(j)}$ is a basis vector, all the elements of $\matcol{A}{j}$ are zero except the $\pi(j)$-th element, which is $\vecentry{u}{j}$. So, for each $j$-th column, $\matentry{A}{\pi(j)}{j}=\vecentry{u}{j}$ is the only non-zero element. Also, since $\pi$ is a permutation, the position of the non-zero element of each column is distinct, i.e., $\matentry{A}{\pi(j)}{j}$ is the only non-zero element in $\pi(j)$-th row of the matrix $\mat{A}.$ Hence, for each $j$, $\matentry{A}{\pi(j)}{j}=\vecentry{u}{j}$ is the only non-zero element of $\pi(j)$-th row as well as $j$-th column of $\mat{A}$.\\

\noindent\textbf{Property 2: }The transpose of the matrix $\mat{A}$ is given by 
    $$\mat{A}^{T}=(\vecentry{u}{\pi^{-1}(0)}\basisvec{\pi^{-1}(0)}~|~\cdots~|~\vecentry{u}{\pi^{-1}(n-1)}\basisvec{\pi^{-1}(n-1)})$$

Enough to show that the $j$-th column of $\mat{A}^{T}$ is $\vecentry{u}{\pi^{-1}(j)}\basisvec{\pi^{-1}(j)}$. Now, the $j$-th column of $\mat{A}^{T}$ = $j$-th row of $\mat{A}$. From the property 1, we know that $\matentry{A}{j}{\pi^{-1}(j)}=\vecentry{u}{\pi^{-1}(j)}$ is the only non-zero element in the $j$-th row as well as $\pi^{-1}(j)$-th column of $\mat{A}$ i.e., the $j$-th row of $\mat{A}$ is, $\matrow{A}{j}=\vecentry{u}{\pi^{-1}(j)}\basisvec{\pi^{-1}(j)}$. Therefore, the $j$-th column of $\mat{A}^{T}=\vecentry{u}{\pi^{-1}(j)}\basisvec{\pi^{-1}(j)}$.\\

\noindent\textbf{Property 3: } The multiplication of any matrix $\mat{G}=(\vect{g}_{0}~|~\cdots~|~\vect{g}_{n-1})$, by the monomial matrix $\mat{A}$ is given by
    $$\mat{GA}=(\vecentry{u}{0}\vect{g}_{\pi(0)}~|~\cdots~|~\vecentry{u}{n-1}\vect{g}_{\pi(n-1)})$$
where $\vect{g}_{j}=\matcol{G}{j}$ is the $j$-th column of the matrix $\mat{G}$.\\

Enough to show that the $j$-th column of $\mat{GA}$ is $\vecentry{u}{j}\vect{g}_{\pi(j)}$. Now, the $i,\ j$-th element of $\mat{GA}$ is given by:
$$\matentry{GA}{i}{j}=\sum_{k=0}^{n-1}\matentry{G}{i}{k}\matentry{A}{k}{j}=\matentry{G}{i}{\pi(j)}\matentry{A}{\pi(j)}{j},$$
since $\matentry{A}{\pi(j)}{j}$ is the only non-zero element in the $j$-th column of $\mat{A}$. 
Therefore the $j$-th column of $\mat{GA}$ is given by
$$\matcol{GA}{j}=\matcol{G}{\pi(j)}\matentry{A}{\pi(j)}{j}=\vect{g}_{\pi(j)}\vecentry{u}{j}=\vecentry{u}{j}\vect{g}_{\pi(j)}$$\\

\noindent\textbf{Property 4: }The multiplication of two monomial matrices $\mat{A}$ and $\mat{B}=(\pi',\ \vect{u'})\in M_{n}$ is given by:
    $$\mat{AB}=(\vecentry{u}{\pi'(0)}\vecentry{u'}{0}\basisvec{\pi(\pi'(0))}~|~\cdots~|~\vecentry{u}{\pi'(n-1)}\vecentry{u'}{n-1}\basisvec{\pi(\pi'(n-1))})$$
    
Enough to show that the $j$-th column of $\mat{AB}$ is $\vecentry{u}{\pi'(j)}\vecentry{u'}{j}\basisvec{\pi(\pi'(j))}$. From the property 3, we have the $j$-th column of $\mat{AB}$ is given by:
$$\matcol{AB}{j}=\vecentry{u'}{j}\matcol{A}{\pi'(j)}$$
Since the $j$-th column of $\mat{A}$ is $\matcol{A}{j}=\vecentry{u}{j}\basisvec{\pi(j)}$, therefore the $\pi'(j)$-th column of $\mat{A}$ will be $\matcol{A}{\pi'(j)}=\vecentry{u}{\pi'(j)}\basisvec{\pi(\pi'(j))}$. Hence, the $j$-th column of $\mat{AB}$ will be 
$\vecentry{u}{\pi'(j)}\vecentry{u'}{j}\basisvec{\pi(\pi'(j))}$.\\

\noindent\textbf{Property 5: } The multiplication of a monomial matrices $\mat{A}$ by a partial monomial matrix $\mat{C}=(\pi_{*},\ \vect{v})\in M_{k}'$ is given by:
    $$\mat{AC}=(\vecentry{u}{\pi_{*}(0)}\vecentry{v}{0}\basisvec{\pi(\pi_{*}(0))}~|~\cdots~|~\vecentry{u}{\pi_{*}(k-1)}\vecentry{v}{k-1}\basisvec{\pi(\pi_{*}(k-1))})$$

Similar to property 4.
\iffalse
Let $\mat{G}=(\vect{g}_{0}~|~\vect{g}_{1}~|~\cdots~|\vect{g}_{n-1})$ be a matrix of order $k\times n$ and $\mat{A}=(\pi,\ \vect{u})\in M_{n}$. Then, the following properties holds: %$\mat{B}=(\pi',\ \vect{u'})\in M_{n}$, $\mat{C}=(\pi_{*},\ \vect{v})\in M_{k}'$. Then the important computational actions of monomial matrices are as follows: 

\begin{enumerate}
    \item $\matentry{A}{\pi(j)}{j}=\vecentry{u}{j}$ is the only non-zero element of $\pi(j)$-th row as well as $j$-th column of $\mat{A}$.\label{properties:Non-zeroElement}
    \item The transpose of the matrix $\mat{A}$ is given by 
    $$\mat{A}^{T}=(\vecentry{u}{\pi^{-1}(0)}\basisvec{\pi^{-1}(0)}~|~\cdots~|~\vecentry{u}{\pi^{-1}(n-1)}\basisvec{\pi^{-1}(n-1)})$$\label{properties:Transpose}
    \item The matrix $\mat{GA}$ is given by
    $$\mat{GA}=(\vecentry{u}{\pi(0)}\vect{g}_{\pi(0)}~|~\cdots~|~\vecentry{u}{\pi(n-1)}\vect{g}_{\pi(n-1)})$$\label{properties:Multiplication}
    \item The multiplication of two monomial matrices $\mat{A}$ and $\mat{B}=(\pi',\ \vect{u'})\in M_{n}$ is given by:
    $$\mat{AB}=(\vecentry{u}{\pi'(0)}\vecentry{u'}{0}\basisvec{\pi(\pi'(0))}~|~\cdots~|~\vecentry{u}{\pi'(n-1)}\vecentry{u'}{n-1}\basisvec{\pi(\pi'(n-1))})$$\label{properties:Mono-Multiplication}
    \item The multiplication of a monomial matrices $\mat{A}$ by a partial monomial matrix $\mat{C}=(\pi_{*},\ \vect{v})\in M_{k}'$ is given by:
    $$\mat{AC}=(\vecentry{u}{\pi_{*}(0)}\vecentry{v}{0}\basisvec{\pi(\pi_{*}(0))}~|~\cdots~|~\vecentry{u}{\pi_{*}(k-1)}\vecentry{v}{k-1}\basisvec{\pi(\pi_{*}(k-1))})$$\label{properties:Mono-PartialMono-Multiplication}
\end{enumerate}
\fi

==> Appendices/Protocols.tex <==
\section{Some interacting protocols}\label{appendix:protocols}
Here the parameters $q,\ n,\ k \in \mathbb{N}$, matrix $\mat{G}_{0} \in \fieldmat{F}{q}{k}{n}$ and
a hash function $\texttt{H}$ are public. The private key for the prover is a monomial matrix $\mat{Q}\in M_{n}$ and the public key is $\mat{G}_{1}=\texttt{RREF}(\mat{G}_{0}\mat{Q}^{-T})$. The interaction between the prover and the verifier is described in the protocol in Fig.~\ref{fig:Sigma_protocol}. 

\begin{figure}[!ht]
%\centering
\includegraphics[width=1\linewidth]{Images/Sigma_Protocol1.pdf}
\caption{LESS-v1 identification scheme~\cite{LESS_is_More}. }
\label{fig:Sigma_protocol}  
\end{figure}

\noindent\textbf{Completeness: } To check the completeness of the protocol, it is to show that for a valid $(\text{cmt,\ ch,\ rsp})$ is always accepted $i.e.$, $\texttt{H}(\texttt{RREF}(\mat{G}_{\text{ch}}\cdot \text{rsp}))$ will be equal to $\text{cmt}$. If \texttt{H} is a collision-resistant hash function, then it is enough to show that for any $\text{ch}\in \left\{0,\ 1\right\}$, $\texttt{RREF}(\mat{G}_{\text{ch}}\cdot \text{rsp})=\widetilde{\mat{G}}$.
\begin{itemize}
    \item \textbf{Case 1: }For $\text{ch}=0$, $\text{rsp}=\widetilde{\mat{Q}}^{T}$. In this case, $\texttt{RREF}(\mat{G}_{\text{ch}}\cdot \text{rsp}))=\texttt{RREF}(\mat{G}_{0}\cdot \widetilde{\mat{Q}}^{T}) = \widetilde{\mat{G}}.$
    
    \item \textbf{Case 2: }For $\text{ch}=1$, $\text{rsp}=\mat{Q}^{T}\widetilde{\mat{Q}}^{T}$, so in this case, $\texttt{RREF}(\mat{G}_{\text{ch}}\cdot \text{rsp}))=\texttt{RREF}(\mat{G}_{1}\cdot \mat{Q}^{T}\widetilde{\mat{Q}}^{T}).$ Since $\mat{G}_{1}=\texttt{RREF}(\mat{G}_{0}\mat{Q}^{-T})$, there exists a non-singular matrix $\mat{E}$ such that $\mat{G}_{1}=\mat{EG}_{0}\mat{Q}^{-T}$. Hence, $$\texttt{RREF}(\mat{G}_{1}\cdot \mat{Q}^{T}\widetilde{\mat{Q}}^{T})=\texttt{RREF}(\mat{EG}_{0}\mat{Q}^{-T}\cdot\mat{Q}^{T} \widetilde{\mat{Q}}^{T})=\texttt{RREF}(\mat{EG}_{0}\widetilde{\mat{Q}}^{T})$$
     Also, since $\widetilde{\mat{G}}=\texttt{RREF}(\mat{G}_{0}\widetilde{\mat{Q}}^{T})$, there exists a non-singular matrix $\mat{E}'$ such that $\widetilde{\mat{G}}=\mat{E}'\mat{G}_{0}\widetilde{\mat{Q}}^{T}$. We can write $\widetilde{\mat{G}}$ as $$\widetilde{\mat{G}}=\mat{E}'\mat{G}_{0}\widetilde{\mat{Q}}^{T}=\mat{E}'\mat{E}^{-1}(\mat{E}\mat{G}_{0}\widetilde{\mat{Q}}^{T})$$ Since $\widetilde{\mat{G}}$ is in $\texttt{RREF}$ and the $\texttt{RREF}$ of a matrix is unique, therefore $\texttt{RREF}(\mat{EG}_{0}\widetilde{\mat{Q}}^{T})=\widetilde{\mat{G}}$.
     So, for $\text{ch}=1$, $\texttt{RREF}(\mat{G}_{\text{ch}}\cdot \text{rsp})=\texttt{RREF}(\mat{EG}_{0}\widetilde{\mat{Q}}^{T})=\widetilde{\mat{G}}$. 
\end{itemize}
Therefore, for any $\text{ch}\in \left\{0,\ 1\right\}$, $\texttt{RREF}(\mat{G}_{\text{ch}}\cdot \text{rsp})=\widetilde{\mat{G}}$, hence, proves that protocol is correct. Also in the protocol in Fig.~\ref{fig:Sigma_protocol}, an honest verifier achieves no information about the secret. This assertion follows from the next Lemma.

\begin{lemma}
For any $\mat{Q}\in M_{n}$ and $\widetilde{\mat{Q}}\xleftarrow[]{\$}M_{n}$, the multiplication matrix $\mat{Q}^{T}\widetilde{\mat{Q}}^{T}$ follows a uniform distribution over the set $M_{n}$~\cite{LESS_is_More}. 
\end{lemma}
When $\text{ch} = 0$, the verifier receives $\text{rsp}=\widetilde{\mat{Q}}^{T}$ as a response, which does not reveal any information about the secret matrix $\mat{Q}$. Similarly, when $\text{ch} = 1$, the verifier gets $\mat{Q}^{T}\widetilde{\mat{Q}}^{T}$ as a response, and since this matrix is uniformly distributed over $M_{n}$, the verifier gains no information about $\mat{Q}$. This holds in either case, ensuring that the verifier remains completely unaware of the secret matrix $\mat{Q}$.\\

\noindent\textbf{Soundness: }The protocol in Fig. ~\ref{fig:Sigma_protocol} is 2-special sound $i.e.$ if we are given two valid transcripts $\text{tr}_{0}=(\text{cmt},\ \text{ch}=0,\ \text{rsp}= \widetilde{\mat{Q}}^{T})$ and $\text{tr}_{1}=(\text{cmt},\ \text{ch}=1,\ \text{rsp}=\mat{Q}^{T}\widetilde{\mat{Q}}^{T})$, then we can find the witness $\mat{Q}$. Next, we calculate the soundness error of this protocol. Let the dishonest prover Eve makes two transcripts as $\text{tr}_{0}=(\text{cmt},\ \text{ch}=0,\ \text{rsp}= \widetilde{\mat{Q}}^{T})$ and $\text{tr}_{1}=(\text{cmt},\ \text{ch}=1,\ \text{rsp}={\mat{Q}}^{*})$, where $\text{cmt}=\texttt{H}(\texttt{RREF}(\mat{G}_{0}\widetilde{\mat{Q}}^{T}))$ and $\mat{Q}^{*}\xleftarrow[]{\$}M_{n}$. Then 
\begin{align*}
    &Pr[\text{Eve will win}]\\
    &=Pr[\text{ch}=0]\cdot Pr[\text{tr}_{0} \text{ is satisfied}~|~\text{ch}=0]+Pr[\text{ch}=1]\cdot Pr[\text{tr}_{1} \text{ is satisfied}~|~\text{ch}=1]\\
    &=\frac{1}{2} (Pr[\text{tr}_{0} \text{ is satisfied}~|~\text{ch}=0]+ Pr[\text{tr}_{1} \text{ is satisfied}~|~\text{ch}=1])
\end{align*}
Now, for the first transcript $\text{tr}_{0}$, $\texttt{H}(\texttt{RREF}(\mat{G}_{\text{ch}}\cdot \text{rsp}))=\texttt{H}(\texttt{RREF}(\mat{G}_{0}\cdot \widetilde{\mat{Q}}^{T}))=\text{cmt}.$ So if $\text{ch}=0$, then the transcript $\text{tr}_{0}$ will always satisfies. Hence, $Pr[\text{tr}_{0} \text{ is satisfied}~|~\text{ch}=0]=1.$ But, if $\text{ch}=1$, then the transcript $\text{tr}_{1}$ will be satisfied if Eve selects the matrix $\mat{Q}^{*}$ as response such that $\texttt{H}(\texttt{RREF}(\mat{G}_{1}\mat{Q}^{*}))=\text{cmt}=\texttt{H}(\texttt{RREF}(\mat{G}_{0} \widetilde{\mat{Q}}^{T})).$ Since $\texttt{H}$ is collision resistant hash function, therefore
\begin{align*}
   \texttt{RREF}(\mat{G}_{1}\mat{Q}^{*})&=\texttt{RREF}(\mat{G}_{0}\widetilde{\mat{Q}}^{T})\\
   \implies \mat{G}_{1} \mat{Q}^{*}&=\mat{SG}_{0} \widetilde{\mat{Q}}^{T}, \text{ for some }\mat{S}\in \text{GL}_{k}\implies \mat{G}_{1}=\mat{SG}_{0} \widetilde{\mat{Q}}^{T}\mat{Q}^{*-1}
\end{align*}
   So, here the prover has to find the monomial matrix $\mat{Q}^{*}$ and a non-singular matrix $S$ such that the previous equation $\mat{G}_{1}=\mat{SG}_{0} \widetilde{\mat{Q}}^{T}\mat{Q}^{*-1}$ holds, and this is the computational version of linear code equivalence problem, which assume to be hard. Therefore, $Pr[\text{tr}_{1} \text{ is satisfied}~|~\text{ch}=1]=\epsilon$, where $\epsilon<<1$. Hence, $
    Pr[\text{Eve will win}]\sim \frac{1}{2}$. \\
    
One can observe that for a dishonest prover, the verifier accepts the response with probability atleast $\frac{1}{2}$. This implies that the soundness error of this identification protocol is atleast $\frac{1}{2}$. However, this protocol can be repeated multiple times to reduce this soundness error. The protocol in Fig.~\ref{fig:Canonical_Identification} reduces the soundness error from $\frac{1}{2}$ to $\frac{1}{2^{st}}$, where $s-1$ is the number of secret monomial matrices and $t$ is the size of the $\text{ch}$ array. This is the modified version of the protocol in Fig.~\ref{fig:Sigma_protocol}.

\begin{figure}[h]
%\centering
\includegraphics[width=1\linewidth]{Images/Sigma_Protocol_update1.pdf}
\caption{The canonical LESS-v1 identification scheme~\cite{LESS_is_More}. }
\label{fig:Canonical_Identification}  
\end{figure}
\begin{figure}[h]
%\centering
\includegraphics[width=1\linewidth]{Images/Final_Less.pdf}
\caption{Final version of LESS. }
\label{fig:Less_final}  
\end{figure}
\begin{lemma}\label{lemma:Less_final}
    The response from an honest prover in the protocol in Fig.~\ref{fig:Less_final}, is always accepted by the verifier.  
\end{lemma}

\begin{proof}
If $\text{ch}_{j}=0$, then clearly $\overline{\mat{V}}_{j}=\overline{\mat{V}}_{j}'$ holds. Now, our goal is to demonstrate that for $\text{ch}_{j}\neq 0$, $\overline{\mat{V}}_{j}=\overline{\mat{V}}_{j}'$ holds.
Let $\mat{Q}_{\text{ch}_{j}}^{T}=(\pi,\ \vect{v})$ and $\widetilde{\mat{Q}}_{j}^{T}=(\pi',\ \vect{v}')$ be two monomial matrices. Consider $\mat{G}_{0}=(\vect{g}_{0}|\vect{g}_{1}|\cdots|\vect{g}_{n-1})$ as the generator matrix where each $\vect{g}_{i}=\mat{G}_{0}[*, i]$ is the $i$-th column of the matrix $\mat{G}_{0}$. Define $\mat{G}_{\text{ch}_{j}}=\texttt{RREF}(\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T})$ and $\widetilde{\mat{G}}_{j}=\texttt{RREF}(\mat{G}_{0}\widetilde{\mat{Q}}_{j}^{T})$.
Let $\mat{G}=\mat{G}_{0}\widetilde{\mat{Q}}_{j}^{T}$ and $J$ be the information set of the code $\mat{G}$. Then, $\widetilde{\mat{G}}_{j}=\matcol{G}{J}^{-1}\mat{G}=\matcol{G}{J}^{-1}\mat{G}_{0}\widetilde{\mat{Q}}_{j}^{T}$ holds. This implies, \begin{align*}
   & \widetilde{\mat{G}}_{j}[*,\ J^{c}]=\matcol{G}{J}^{-1}\mat{G}_{0}\widetilde{\mat{Q}}_{j}^{T}[*,\ J^{c}]
\end{align*}
Now the $i$-column of the matrix $\mat{G}_{0}\widetilde{\mat{Q}}_{j}^{T}[*,\ J^{c}]$ is given by $\vecentry{v'}{j_{i}}\vect{g}_{\pi'(j_{i})}$, where $j_{i}$ is the $i$-th element of the ordered set $J^{c}$.
Therefore, the matrix $\widetilde{\mat{G}}_{j}[*,\ J^{c}]$ will be $\widetilde{\mat{G}}_{j}[*,\ J^{c}]=(\vecentry{v'}{j_{0}}\matcol{G}{J}^{-1}\vect{g}_{\pi'(j_{0})}~|~\cdots~|~\vecentry{v'}{j_{k-1}}\matcol{G}{J}^{-1}\vect{g}_{\pi'(j_{k-1})})$, for all $j_{i}\in J^{c}$.
Considering that $\vecentry{v'}{j_{i}}$ is a non-zero scalar, for all $j_{i}\in J^{c}$, we have:
\begin{align*}
        &\texttt{LexMinCol}(\vecentry{v'}{j_{i}}\matcol{G}{J}^{-1}\vect{g}_{\pi'(j_{i})})
        =\texttt{LexMinCol}(\matcol{G}{J}^{-1}\vect{g}_{\pi'(j_{i})})\\
    \implies &\texttt{LexMinCol}(\widetilde{\mat{G}}_{j}[*,\ J^{c}])
        =\texttt{LexMinCol}(\mat{B})
\end{align*}
where $\matcol{G}{J}^{-1}\vect{g}_{\pi'(j_{i})}$ is the $i$-th column of the matrix $\mat{B}$. Therefore, $$\overline{\mat{V}}_{j}=\texttt{LexSort}(\texttt{LexMinCol}(\widetilde{\mat{G}}_{j}[*,\ J^{c}]))=\texttt{LexSort}(\texttt{LexMinCol}(B))$$
To prove $\overline{\mat{V}}_{j}=\overline{\mat{V}}_{j}'$, it suffices to demonstrate that each column of $\widetilde{\mat{G}}_{j}'[*, J'']$ is a non-zero scaler multiple of some column of $\mat{B}$. Considering the relationship $\mat{Q}_{\text{ch}_{j}}^{T}\overline{\mat{Q}}_{j}=\mat{Q}_{\text{ch}_{j}}^{T}\widetilde{\mat{Q}}_{j}^{T}[*,\ J]$, we obtain $J'=\ring{Z}{n}\setminus\left\{\pi(\pi'(j)): j\in J\right\}=\left\{\pi(\pi'(j)): j\in J^{c}\right\}$, representing the positions of zero rows in the matrix $\mat{Q}_{\text{ch}_{j}}^{T}\overline{\mat{Q}}_{j}$.
Now, $\mat{P}=\mat{G}_{\text{ch}_{j}}\cdot \text{rsp}_{j}=\mat{G}_{\text{ch}_{j}}\cdot \mat{Q}_{\text{ch}_{j}}^{T}\overline{\mat{Q}}_{j}$ and $\mat{R}=\mat{G}_{\text{ch}_{j}}[*, J']$. Since $\mat{G}_{\text{ch}_{j}}=\texttt{RREF}(\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T})$, therefore there exists a matrix $\mat{S}\in GL_{k}(q)$ such that $\mat{G}_{\text{ch}_{j}}=\mat{SG}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}$. Therefore,
\begin{align*}
&\mat{P}=\mat{S}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}\cdot \mat{Q}_{\text{ch}_{j}}^{T}\overline{\mat{Q}}_{j}=\mat{S}\mat{G}_{0}\overline{\mat{Q}}_{j} \text{ and }
\mat{R}=\mat{S}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}[*,\ J']
\end{align*}
Now,
\begin{align*}
\widetilde{\mat{G}}_{j}'&=\texttt{RREF}\left(\mat{P}~|~\mat{R}\right)=\texttt{RREF}(\mat{S}\mat{G}_{0}\overline{\mat{Q}}_{j}~|~\mat{S}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}[*,\ J'])=\texttt{RREF}(\mat{G}_{0}\overline{\mat{Q}}_{j}~|~\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}[*,\ J'])\\
&=\texttt{RREF}(\matcol{G}{J}~|~\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}[*,\ J'])=(\mathbf{I}_{k}~|~\matcol{G}{J}^{-1}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}[*,\ J']),
\end{align*}
since $J$ is the information set of $\mat{G}$. Therefore 
$\widetilde{\mat{G}}_{j}'[*,\ J'']=\matcol{G}{J}^{-1}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}^{-T}[*,\ J']$. Therefore, each column of $\widetilde{\mat{G}}_{j}'[*,\ J'']$ is a multiple of the term $\matcol{G}{J}^{-1}\vect{g}_{\pi^{-1}(j')}$, where $j'\in J'$. Since $J'=\left\{\pi(\pi'(j')):j'\in J^{c}\right\}$, each column of $\widetilde{\mat{G}}_{j}'[*,\ J'']$ is a multiple of $\matcol{G}{J}^{-1}\vect{g}_{\pi'(j_{i})}$, where $j_{i}\in J^{c}$. Thus, $\overline{\mat{V}}_{j}'=\texttt{LexSort}(\mat{B})=\overline{\mat{V}}_{j}$.
The completeness of the protocol illustrated in Fig.~\ref{fig:Less_final} is established.

\end{proof}




\iffalse
\begin{proof}
If $\text{ch}_{j}=0$, then clearly $\overline{\mat{V}}_{j}=\overline{\mat{V}}_{j}'$ holds. Now, our goal is to demonstrate that for $\text{ch}_{j}\neq 0$, $\overline{\mat{V}}_{j}=\overline{\mat{V}}_{j}'$ holds.
Let $\mat{Q}_{\text{ch}_{j}}^{-1}=(\pi,\ \vect{v})$ and $\widetilde{\mat{Q}}_{j}=(\pi',\ \vect{v}')$ be two monomial matrices. Consider $\mat{G}_{0}=(\vect{g}_{0}|\vect{g}_{1}|\cdots|\vect{g}_{n-1})$ as the generator matrix where each $\vect{g}_{i}=\mat{G}_{0}[*, i]$ is the $i$-th column of the matrix $\mat{G}_{0}$. Define $\mat{G}_{\text{ch}_{j}}=\texttt{RREF}(\mat{G}_{0}\mat{Q}_{\text{ch}_{j}})$ and $\widetilde{\mat{G}}_{j}=\texttt{RREF}(\mat{G}_{0}\widetilde{\mat{Q}}_{j})$.
Let $\mat{G}=\mat{G}_{0}\widetilde{\mat{Q}}{j}$ and $J$ be the information set of the code $\mat{G}$. Then, $\widetilde{\mat{G}}_{j}=\matcol{G}{J}^{-1}\mat{G}=\matcol{G}{J}^{-1}\mat{G}_{0}\widetilde{\mat{Q}}_{j}$
\begin{align*}
    &\widetilde{\mat{G}}_{j}=\matcol{G}{J}^{-1}\mat{G}=\matcol{G}{J}^{-1}\mat{G}_{0}\widetilde{\mat{Q}}_{j}
\end{align*}
Since $\mat{G}_{\text{ch}_{j}}=\texttt{RREF}(\mat{G}_{0}\mat{Q}_{\text{ch}_{j}})$, therefore there exists a non-singular matrix $S$ of order $k$ such that
\begin{align*}
&\mat{G}_{\text{ch}_{j}}=\mat{SG}_{0}\mat{Q}_{\text{ch}_{j}}
\end{align*}
Now,
\begin{align*}
   & \widetilde{\mat{G}}_{j}[*,\ J^{c}]=\matcol{G}{J}^{-1}\mat{G}_{0}\widetilde{\mat{Q}}_{j}[*,\ J^{c}]
\end{align*}
So, the set of columns of the matrix $\widetilde{\mat{G}}_{j}[*,\ J^{c}]$ is given by 
\begin{align*}
    &A=\left\{\vecentry{v'}{j}\matcol{G}{J}^{-1}\vect{g}_{\pi'(j)}:~j\in J^{c}\right\}
\end{align*}
Considering that $\vecentry{v'}{j}$ is a scalar, for all $j\in J^{c}$, we have:
\begin{align*}
    &\texttt{LexMinCol}(\vecentry{v'}{j}\matcol{G}{J}^{-1}\vect{g}_{\pi'(j)})
    =\texttt{LexMinCol}(\matcol{G}{J}^{-1}\vect{g}_{\pi'(j)})
\end{align*}
Therefore, $\overline{\mat{V}}_{j}=\texttt{LexSort}(B)$, where 
\begin{align*}
&B=\left\{LexMinCol(\matcol{G}{J}^{-1}\vect{g}_{\pi'(j)}):~j\in J^{c}\right\}    
\end{align*}
To prove $\overline{\mat{V}}_{j}=\overline{\mat{V}}_{j}'$, it suffices to demonstrate that each column of $\widetilde{\mat{G}}_{j}'[*, J'']$ is a multiple of some column of $B$.

Considering the relationship
\begin{align*}
&\mat{Q}_{\text{ch}_{j}}^{-1}\overline{\mat{Q}}_{j}=\mat{Q}_{\text{ch}_{j}}^{-1}\widetilde{\mat{Q}}_{j}[*,\ J]
\end{align*}
we obtain $J'=\ring{Z}{n}\setminus\left\{\pi(\pi'(j)): j\in J\right\}=\left\{\pi(\pi'(j)): j\in J^{c}\right\}$, representing the positions of zero rows in the matrix $\mat{Q}_{\text{ch}_{j}}^{-1}\overline{\mat{Q}}_{j}$.
Now,
\begin{align*}
&\mat{P}=\mat{G}_{\text{ch}_{j}}\cdot \text{rsp}_{j}=\mat{S}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}\cdot \mat{Q}_{\text{ch}_{j}}^{-1}\overline{\mat{Q}}_{j}=\mat{S}\mat{G}_{0}\overline{\mat{Q}}_{j}\\
&\mat{R}=\mat{G}_{\text{ch}_{j}}[*, J']=\mat{S}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}[*,\ J']\\
&\widetilde{\mat{G}}_{j}'=\texttt{RREF}\left((\mat{P}~|~\mat{R})\right)\\
&=\texttt{RREF}\left((\mat{S}\mat{G}_{0}\overline{\mat{Q}}_{j}~|~\mat{S}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}[*,\ J'])\right)\\
&=(\mathbf{I}_{k}~|~\matcol{G}{J}^{-1}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}[*,\ J'])\\
&\widetilde{\mat{G}}_{j}'[*,\ J'']=\matcol{G}{J}^{-1}\mat{G}_{0}\mat{Q}_{\text{ch}_{j}}[*,\ J']
\end{align*}
Therefore, each column of $\widetilde{\mat{G}}_{j}'[*,\ J'']$ is a multiple of the term $\matcol{G}{J}^{-1}\vect{g}_{\pi^{-1}(j)}$, where $j\in J'$. Since $J'=\left\{\pi(\pi'(j)):j\in J^{c}\right\}$, each column of $\widetilde{\mat{G}}_{j}'[*,\ J'']$ is a multiple of $\matcol{G}{J}^{-1}\vect{g}_{\pi^{-1}(j)}$, where $j\in J^{c}$. Thus, $\overline{\mat{V}}_{j}'=\texttt{LexSort}(B)=\overline{\mat{V}}_{j}$.
The completeness of the protocol illustrated in Fig.~\ref{fig:Less_final} is established.
\end{proof}
\fi

==> Sections/test.tex <==
\subsection{Attack template}\label{sec:attackTemplate}
In this section, first, we will describe how to obtain the secret monomial matrices from an effective faulted signature $\tau=(salt,\ cmt,\ \vect{Tree Node},\ \vect{rsp})$ in Alg.~\ref{alg:RecoverSecret}. Let $\vecentry{x}{i}$ be the node in \textit{Reference Tree} with height $h$, and $L_{\vecentry{x}{i}}$ be the set of all leaf nodes of the subtree rooted at $\vecentry{x}{i}$. We only need the leaf nodes from $L_{\vecentry{x}{i}}$ that coincide with the first $t$ many leaf nodes of the full \textit{Reference Tree}. Without loss of generality, assume that there are $v$ many such leaves, and let the set of indices of these leaves be 
$$I^{(i)}_{\text{leaf}} = \{j_1,\ j_2,\ \cdots,\ j_v\}\,.$$
%Therefore, the values of the vector $\vect{f}$ and the digest vector $\vect{d}$ corresponding to the set of indices $I_{\text{leaf}}^{(i)}$ will be $\left\{\vecentry{f}{j_{1}-2l+1},\ \cdots,\ \vecentry{f}{j_{v}-2l+1}\right\}$ and $\left\{\vecentry{d}{j_{1}-2l+1},\ \cdots,\ \vecentry{d}{j_{v}-2l+1}\right\}$ respectively. 
As we discussed before, from this effective faulted signature, the information of columns of all the secret matrices $\mat{Q}_{\vecentry{d}{j-2l+1}}^{T}$  will be recovered with Alg.~\ref{alg:RecoverSecret}, where $j\in I_{\text{leaf}}^{(i)}$ and $\vecentry{d}{j-2l+1}\neq 0$.
% Next, we will discuss the exact scenario of our attack.

\begin{algorithm}
\caption{\texttt{Recover\_Secret\_Matrices}($\tau,\ PK$)}\label{alg:RecoverSecret}
\begin{algorithmic}[1]
\Require Signature $\tau=(\textit{salt},\ \textit{cmt},\ \vect{TreeNode},\ \vect{rsp})$, public key $PK=(gseed,\ \mat{G}_{1},\ \cdots,\ \mat{G}_{s-1})$.
\Ensure The columns of secret matrices $\mat{Q}_{\vecentry{d}{j-2l+1}}^{T}$, where $j\in I_{\text{leaf}}^{(i)}$ and $\vecentry{d}{j-2l+1}\neq 0$.

\State $\vect{d}\leftarrow \texttt{CSPRNG}(cmt,\ \mathbb{S}_{t,w})$
\State $\vect{seed}\leftarrow \texttt{SeedTreeUpdate}(\vect{TreeNode},\ salt)$
\State $\vect{ESEED}\leftarrow $ Leaf nodes of $\vect{seed}$ corresponding to $\vecentry{seed}{i}$
\State $\mat{G}_{0}\leftarrow \texttt{CSPRNG}(gseed,\ \mathbb{S}_{\texttt{RREF}})$

\For{$r=1;\ r\leq v;\ r=r+1$}
    \If{$\vecentry{d}{j_{r}-2l+1}\neq 0$}
       \State $\widetilde{\mat{Q}}_{j_{r}-2l+1}\leftarrow \texttt{CSPRNG}(\vecentry{ESEED}{j_{r}-2l+1},\ \vect{M}_{n})$
       \State $(\overline{\mat{Q}}_{j_{r}-2l+1},\ \overline{\mat{V}}_{j_{r}-2l+1})\leftarrow \texttt{PrepareDigestInput}(\mat{G}_{0},\ \widetilde{\mat{Q}}_{j_{r}-2l+1})$
       \State $\mat{Q}^{*}=\mat{Q}_{\vecentry{d}{j_{r}-2l+1}}^{T}\overline{\mat{Q}}_{j_{r}-2l+1}\leftarrow \texttt{ExpandToMonomAction}(\vect{rsp})$ 
       \State Compute $\mat{Q}_{\vecentry{d}{j_{r}-2l+1}}^{T}\leftarrow(\mat{Q}^{*},\ \overline{\mat{Q}}_{j_{r}-2l+1})$ \Comment{following Lemma~\ref{lemma:partial_monomial}}
        \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

Here \texttt{SeedTreeUpdate} function takes the $\vect{TreeNode}$, \textit{salt} and digest $\vect{d}$ and generates all the ephemeral seeds assuming the modified \textit{Reference Tree} after effective fault. Since $\vecentry{seed}{i}$ is revealed in $\vect{TreeNode}$ after effective fault, we can say that $\vecentry{ESEED}{j-2l+1}$ for all $j\in I_{\text{leaf}}^{(i)}$ are revealed.
%Here \texttt{SeedTreeUpdate} is the restricted part of the function \texttt{SeedTree}, that is used to generate all the leaf seeds corresponding to the seed $\vecentry{seed}{i}$.

Assume that we are able to get into the victim's device and introduce the fault that causes it to bypass the $Ins(i)$ instruction. The \texttt{LESS\_KeyGen} Alg.~\ref{alg:KeyGen} is a one-time operation from where the secret key $SK=( MSSED,\ gseed)$ and public key $PK=(gseed,\ \mat{G}_{1},\ \cdots,\ \mat{G}_{s-1})$ are generated. But with this private key $SK$, the \texttt{LESS\_Sign} Alg.~\ref{alg:Signature} can execute more than once. We follow the following subsequent actions to find the secret monomial matrices:
\begin{enumerate}
    \item We request for a message, signature pair $(m,\ \tau)$ to the victim device.
    \item After receiving the pair $(m,\ \tau)$, we will determine whether or not $\tau$ is an effective faulted signature. Go back to step 1 if the signature is not effective. If yes, then go to the next step.
    \item Using this signature $\tau$, we will run the \texttt{Recover\_Secret\_Matrices} Alg.~\ref{alg:RecoverSecret} to determine the hidden monomial matrices.
    \item Next, we will calculate whether or not the whole secret monomial matrices were obtained. We stop if the secret matrices are recovered. If not, we repeat the same procedure to retrieve the remaining non-recovered columns. 
\end{enumerate}
